How do standard time series forecasting benchmarks translate to finance? A broad study of risk adjusted performance

Forecasting financial asset returns is challenging due to low signal-to-noise ratios, non-stationarity and heavy-tailed distributions. We benchmark 16 deep learning architectures for time series forecasting, including Transformers, State Space Models (SSMs), xLSTMs and recurrent hybrids, on a 15-year daily futures dataset using an end-to-end volatility-targeted Sharpe ratio optimisation task. Our results challenge prevailing assumptions in the literature. Several widely used 'state-of-the-art' architectures, including generic Transformers and SSMs, underperformed a simple AR(1) benchmark in a realistic financial forecasting task. The strongest results came from comparatively simple hybrid approaches using recurrent structures: a Variable Selection Network combined with an LSTM achieved the highest Sharpe ratio, while xLSTM showed the greatest robustness to transaction costs. These findings suggest that success on standard time-series benchmarks does not reliably transfer to finance, and that architectures tailored to the unique properties of asset returns may remain more effective than generic attention-based approaches for financial forecasting.

==> Sections/disclosure.tex <==
There are no competing interests. No funding was received.

==> Sections/eda.tex <==
% This section documents the empirical properties of the input variables used in the analysis. Understanding the distributional structure of the data is essential both for assessing the adequacy of standard econometric benchmarks and for motivating the use of flexible nonlinear prediction architectures.

% \subsection{Distribution of Daily Returns and Volatility}

% Daily returns exhibit strong deviations from Gaussianity, characterized by heavy tails and excess kurtosis that imply substantial downside risk and state dependence, Figure~\ref{fig:returns_dist}. These properties are well documented in financial markets and pose challenges for linear predictive models.

% Realized volatility displays pronounced skewness and persistent time variation, consistent with volatility clustering and regime shifts, Figure~\ref{fig:volatility_dist}. This motivates modeling approaches that adapt to changing risk conditions.

% To further assess tail behavior, Figure~\ref{fig:qq_logtails} reports a quantile--quantile plot of returns against the normal distribution together with the log-scale distribution of absolute returns. The QQ plot reveals substantial deviations from normality in both tails, while the log-scale plot indicates slow tail decay consistent with heavy-tailed return behavior. These features are particularly relevant for commodity and electricity markets, where supply constraints, storage frictions, and regulatory mechanisms can generate abrupt price adjustments.

% \begin{figure*}[t]
%     \centering
%         \centering
%         \includegraphics[width=\textwidth]{Images/data_vs_normal.png}
%         \caption{Left: Quantile--quantile plot against the normal distribution. Right: Tail behavior of daily returns. The figures indicate substantial deviations from Gaussianity and heavy-tailed return dynamics.}
%     \label{fig:qq_logtails}
% \end{figure*}

% \subsection{Distribution of Predictive Features}

% In contrast to realized returns, the predictive variables derived from past prices and technical indicators display considerably more regular behavior, Figure~\ref{fig:data_mom}. Momentum features computed over multiple horizons, including daily, weekly, monthly, quarterly, semiannual, and annual returns, as well as MACD-based indicators, are approximately symmetric and centered near zero. 

% This relative stability reflects the fact that these predictors are normalized transformations of price dynamics rather than direct measures of realized outcomes. While their distributions are well-behaved, their relationship with future returns is not necessarily linear or constant across states. Consequently, linear combinations of such predictors may fail to capture the conditional nonlinearities through which information is translated into returns.

% Volatility targeting introduces a time-varying exposure component that mechanically amplifies positions in low-volatility regimes and compresses them during periods of elevated risk. This induces nonlinear, state-dependent effects that interact with predictive signals and are not naturally captured by linear specifications.


% \subsection{Implications for Modeling}

% Taken together, the distributional evidence highlights a fundamental feature of the data. While the input predictors are largely bounded, symmetric, and well-behaved, the target variable—realized returns—exhibits extreme kurtosis, heavy tails, and strong state dependence. This mismatch implies that the primary modeling challenge lies not in stabilizing the inputs, but in accurately capturing the conditional distribution of returns given these inputs.

% These empirical properties motivate the use of flexible nonlinear architectures that can accommodate interactions, threshold effects, and regime-dependent behavior. Nonlinear dependencies and regime changes are frequently observed in financial time series and are captured most effectively by nonlinear models \cite{nonlinear_best}.  Neural network architectures such as LSTMs have shown superior performance in capturing complex nonlinear patterns in volatility and return dynamics \cite{nn_for_nonlinear}. In environments where small changes in predictors can, under certain conditions, lead to disproportionately large changes in outcomes, models that adapt their functional form across the state space are particularly well suited. The subsequent sections evaluate the extent to which modern deep learning architectures can exploit these features systematically and economically meaningful manner.


% \section{Exploratory Data Analysis}

This section summarizes the key empirical properties of the data relevant for modeling. Detailed distributional evidence and feature construction procedures are reported in Appendix~\ref{appdx:eda}.

\subsection{Stylized Facts of Returns and Volatility}

Daily returns exhibit strong deviations from Gaussianity, with heavy tails and excess kurtosis that imply substantial downside risk and state dependence. Realized volatility is highly skewed and persistent, reflecting clustering and regime-dependent risk dynamics. These features challenge linear predictive models that rely on homoskedastic or symmetric error assumptions.

\subsection{Predictive Features and Modeling Implications}

In contrast to realized returns, predictive features derived from past prices and technical indicators are well-behaved, approximately symmetric, and bounded. The primary modeling challenge therefore lies not in stabilizing the inputs, but in capturing the nonlinear and state-dependent mapping from predictors to future returns. This motivates the use of flexible nonlinear architectures capable of adapting across regimes.

\subsection{Implications for Modeling}

Taken together, the distributional evidence highlights a fundamental feature of the data. While the input predictors are largely bounded, symmetric, and well-behaved, the target variable—realized returns—exhibits extreme kurtosis, heavy tails, and strong state dependence. This mismatch implies that the primary modeling challenge lies not in stabilizing the inputs, but in accurately capturing the conditional distribution of returns given these inputs.

These empirical properties motivate the use of flexible nonlinear architectures that can accommodate interactions, threshold effects, and regime-dependent behavior. Nonlinear dependencies and regime changes are frequently observed in financial time series and are captured most effectively by nonlinear models \cite{nonlinear_best}.  Neural network architectures such as LSTMs have shown superior performance in capturing complex nonlinear patterns in volatility and return dynamics \cite{nn_for_nonlinear}. In environments where small changes in predictors can, under certain conditions, lead to disproportionately large changes in outcomes, models that adapt their functional form across the state space are particularly well suited. The subsequent sections evaluate the extent to which modern deep learning architectures can exploit these features systematically and economically meaningful manner.

==> Sections/reduced_benchmark.tex <==
\section{Empirical Results}

This section presents a comprehensive evaluation of the out-of-sample performance of the considered models across multiple market regimes, performance metrics, and computational dimensions~\ref{appdx:measures}. We focused on (i) risk-adjusted returns across subperiods, (ii) aggregate return performance and statistical significance, (iii) downside and tail-risk characteristics, (iv) robustness to seed selection and experimental budget, and (v) the trade-off between predictive performance and computational complexity.

\subsection{Data Description}
\label{sec:data_description}

Our empirical analysis was conducted on a diversified cross-asset futures dataset comprising instruments from five asset classes: bonds, commodities, energy, foreign exchange, and equity indices. Daily closing prices were used to construct returns and predictive features. A detailed description of data construction and exploratory analysis is provided in Appendix~\ref{appdx:eda}.

The dataset exhibited several well-documented stylized facts of financial time series, including heavy-tailed return distributions, volatility clustering, and strong deviations from Gaussianity. These properties are illustrated formally in Appendix~\ref{appdx:eda}, where we report distributional diagnostics (e.g., QQ-plots) and volatility dynamics. As such, the dataset constituted a realistic and challenging benchmark for evaluating nonlinear forecasting architectures in a cross-asset setting.

Although the empirical evidence was robust within our cross-asset benchmark, the results should be interpreted as conditional on the specific dataset and period considered. Extending the analysis to alternative markets and sampling frequencies would further clarify the external validity of the findings.

\subsection{Performance Across Market Regimes}

Table~\ref{tab:performance_by_period_extended} reported out-of-sample Sharpe ratios across five non-overlapping subperiods spanning 2000–2025, together with several aggregated averages. This regime-wise decomposition allowed us to assess model robustness across heterogeneous market environments, including the pre- and post-Global Financial Crisis (GFC), the relatively low-volatility period of the 2010s, and the structurally distinct post-2020 regime characterized by elevated macroeconomic and market volatility.

Several important patterns emerged.

First, deep nonlinear models consistently outperformed linear benchmarks on average. This finding was consistent with the view that purely linear dynamics were insufficient to fully capture the complex and non-stationary structure of financial time series in our dataset. That said, linear models such as AR(1), AR($n$), DLinear, and NLinear achieved Sharpe ratios above one in the most recent subperiod (2020–2025). This observation suggested that short-horizon linear dependencies remained exploitable in high-volatility regimes, where return persistence or rapid mean reversion may temporarily dominate. However, these gains did not generalize across time, and linear models exhibited substantially weaker average performance and limited robustness across regimes.

In contrast, models explicitly designed to learn richer temporal representations exhibited both higher average performance and greater stability across regimes. Among these, SeqRep and the Momentum Transformer achieved the strongest results. The Momentum Transformer obtained the highest overall average Sharpe ratio (2.64), driven primarily by strong performance in earlier subperiods (2000–2010). However, its relative advantage diminished in the post-2015 period, suggesting some sensitivity to structural changes in market behavior.

SeqRep demonstrated comparatively strong temporal consistency. It achieved the highest average Sharpe ratios over both 2010–2025 (2.02) and 2015–2025 (1.91), and maintained stable performance across subperiods. This stability was consistent with the hypothesis that architectures incorporating explicit sequence representations may better accommodate evolving temporal structure and asset-specific dynamics. The superior post-2015 performance suggested a comparatively stronger ability to adapt to changing market conditions within the considered benchmark.

State-space models such as Mamba and Mamba2 exhibited heterogeneous and regime-dependent performance. While computationally efficient, their empirical performance varied considerably across subperiods. Augmenting Mamba2 with a Variable Selection Network (VSN) partially mitigated this instability, suggesting that explicit feature conditioning may be beneficial in low signal-to-noise environments such as financial returns.

Patch-based transformer models, including PatchTST and the hybrid SeqRep+PatchTST, delivered moderate and relatively stable improvements over classical transformer baselines. Nevertheless, their Sharpe ratios remained below those of the strongest sequence representation models, particularly in the post-2015 period. This finding suggested that temporal patching alone was insufficient to address the non-stationarity and low signal-to-noise ratio inherent in financial data without complementary representation learning mechanisms.

xLSTM-based architectures also exhibited stable performance. The xLSTM achieved Sharpe ratios between approximately 1.5 and 2.3 across subperiods, making it one of the more stable performers in the study. This stability suggested that enriching traditional LSTM architectures with matrix-valued states may enhance their ability to model complex temporal dependencies. Augmenting xLSTM with a VSN did not yield systematic performance improvements, indicating that the internal state representation may already capture a substantial portion of the relevant cross-feature structure.

Taken together, these results were consistent with the hypothesis articulated in the introduction: that successful financial forecasting models benefit from denoising mechanisms, asset-specific representation learning, and stable temporal encoding. However, these interpretations remain conditional on the statistical properties of the dataset considered.

\subsection{Aggregate Return Performance and Statistical Significance}
\label{sub:agg_performanc}

Table~\ref{tab:performance_main} reported full-sample out-of-sample performance under a volatility-targeting constraint of 10\%. SeqRep delivered the strongest overall performance across most dimensions, achieving a 23.9\% annualized return with a Sharpe ratio of 2.39. Its HAC-adjusted $t$-statistic of 8.81 indicated strong statistical reliability within the evaluation framework.

When benchmarked against the passive strategy, SeqRep achieved an information ratio of 0.854 and an HAC $t$-statistic relative to passive of 3.31. Its correlation with the passive portfolio (0.404) suggested meaningful diversification benefits.

The hybrid SeqRep+PatchTST attained comparable economic performance (Sharpe 2.32), suggesting that patch-based attention may complement sequential representations. Temporal Fusion Transformer (TFT) also achieved strong performance (Sharpe 2.20), though slightly below SeqRep in both absolute and passive-relative metrics.

Linear benchmarks exhibited Sharpe ratios below one and limited statistical reliability. Their passive-relative metrics were close to zero or negative, and correlations with the passive benchmark were generally higher, suggesting limited incremental explanatory power within this dataset.

Figure~\ref{fig:performance_comparison} visually corroborated these findings. SeqRep-based strategies dominated both gross and net cumulative PnL trajectories, indicating that the observed Sharpe ratios reflected persistent performance rather than isolated episodes.

\subsection{Downside Risk and Tail Behavior}
\label{sub:downside}

Table~\ref{tab:risk_metrics} reported downside and tail-risk metrics.

SeqRep and SeqRep+PatchTST exhibited favorable downside profiles relative to many competing architectures, combining moderate drawdowns with high Calmar ratios. SeqRep achieved comparatively mild worst three-month Sharpe ratios and one of the lowest CVaR levels, suggesting improved tail-risk characteristics within the benchmark.

VSN+xLSTM achieved the lowest maximum drawdown and the highest Calmar ratio, though with somewhat lower average returns than SeqRep. In contrast, standard LSTM and PatchTST architectures experienced larger drawdowns and weaker worst-period performance.

Overall, SeqRep-based models appeared to offer an attractive trade-off between upside performance and downside risk within the dataset considered.

\subsection{Robustness to Seed Selection and Experimental Budget}

Table~\ref{tab:small_seed} evaluated robustness under a substantially reduced experimental budget.

Performance levels and model rankings remained largely stable. SeqRep continued to achieve the strongest risk-adjusted performance (Sharpe 2.40), closely matching its full-budget results. TFT and xLSTM+VSN also retained strong performance, while the AR(1) benchmark remained substantially weaker.

Downside metrics exhibited similar stability. Maximum drawdowns, Calmar ratios, and CVaR levels remained quantitatively consistent with the primary evaluation.

These findings suggested that the relative performance ordering was not primarily driven by extensive seed exploration, but rather reflected structural differences in model architectures within the evaluation framework.

\subsection{Discussion}
\label{sec:discussion}

The empirical findings suggested several consistent patterns regarding inductive biases for financial time-series modeling, conditional on the dataset and evaluation framework considered.

Architectures maintaining explicit or implicit recurrent state representations tended to outperform purely attention-based models across most evaluation dimensions. This pattern was consistent with the view that persistent state representations may be advantageous in environments characterized by regime dependence and autocorrelation.

Hybrid architectures combining structured temporal modeling with feature selection or representation compression achieved the strongest and most stable results. These findings suggested that integrating multiple inductive biases may provide robustness in low signal-to-noise environments.

State-space models demonstrated favorable computational properties but exhibited more heterogeneous empirical performance. The inclusion of explicit feature conditioning partially mitigated this variability.

Linear benchmarks performed reasonably well in specific regimes but did not exhibit robust performance across time, suggesting that short-term linear dependencies may be episodically present but insufficient for consistent forecasting performance.

Taken together, the evidence suggested — rather than conclusively established — that successful financial forecasting architectures benefit from (i) persistent temporal state representations, (ii) adaptive feature conditioning, and (iii) sufficient nonlinear flexibility to accommodate regime-dependent behavior.

\subsection{Computational Efficiency and Model Complexity}

Table~\ref{tab:complexity} compared parameter counts and asymptotic runtime and memory complexity.

Linear models exhibited minimal computational costs but weaker empirical performance. Among nonlinear architectures, SeqRep offered a favorable balance between performance and scalability due to its linear memory complexity in sequence length. Although Mamba and Mamba2 exhibited comparable asymptotic efficiency, their empirical performance was weaker in this benchmark.

Hybrid architectures incurred higher computational costs without uniformly superior performance, raising questions about cost-effectiveness in large-scale or latency-sensitive applications.

Overall, these findings suggested that architectural inductive bias may be more consequential than asymptotic complexity alone when modeling noisy financial time series.

